Analytic energy gradients for variational two-electron reduced-density matrix methods within the density-fitting approximation

Analytic energy gradients are presented for a variational two-electron reduced-density-matrix-driven complete active space self-consistent field (v2RDM-CASSCF) procedure that employs the density-fitting (DF) approximation to the two-electron repulsion integrals. The DF approximation significantly reduces the computational cost of v2RDM-CASSCF gradient evaluation, in terms of both the number of floating-point operations and memory requirements, enabling geometry optimizations on much larger chemical systems than could previously be considered at the this level of theory [E. Maradzike et al., J. Chem. Theory Comput., 2017, 13, 4113-4122]. The efficacy of v2RDM-CASSCF for computing equilibrium geometries and harmonic vibrational frequencies is assessed using a set of 25 small closed- and open-shell molecules. Equilibrium bond lengths from v2RDM-CASSCF differ from those obtained from configuration-interaction-driven CASSCF (CI-CASSCF) by 0.62 pm and 0.05 pm, depending on whether the optimal reduced-density matrices from v2RDM-CASSCF satisfy two-particle N-representability conditions (PQG) or PQG plus partial three-particle conditions (PQG+T2), respectively. Harmonic vibrational frequencies, which are obtained by finite differences of v2RDM-CASSCF analytic energy gradients, similarly demonstrate that quantitative agreement between v2RDM- and CI-CASSCF requires the consideration of partial three-particle N-representability conditions. Lastly, optimized geometries are obtained for the lowest-energy singlet and triplet states of the linear polyacene series up to dodecacene (C50H28), in which case the active space is comprised of 50 electrons in 50 orbitals. The v2RDM-CASSCF singlet-triplet energy gap extrapolated to an infinitely-long linear acene molecule is found to be 7.8 kcal/mol

==> sinfo.tex <==
Supporting information goes here.



==> tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Summary of notation used in theory section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
	\caption{Summary of Notation}
	\label{tab:notation}
	\begin{center}
		{\scriptsize
			\begin{tabular}{l l}
				\hline\hline
				Label & Summary \\
				\hline
				$p,q,r,s$ & general molecular orbitals \\
				$i,j,k,l$ & inactive (doubly occupied) orbitals \\
				$t,u,v,w,x,y$ & active orbitals \\
				$P,Q,R,S$ & auxiliary basis functions \\
				$\sigma,\tau,\kappa,\lambda,\mu,\nu$ & spin functions \\
				PQG & v2RDM-CASSCF subject to the PQG conditions \\
				PQG+T2 & v2RDM-CASSCF subject to the PQG+T2 conditions \\
				\hline\hline
			\end{tabular}
		}
	\end{center}		
	
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% List of molecules, term symbols, and active spaces.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\begin{table}

    \caption{Term symbols and active spaces for the small molecules that 
    comprise our test set.}

    \label{tab:molecules}

    \begin{center}
        {\scriptsize
            \begin{tabular}{l c c }
                \hline\hline
                Molecule & Term & Active Space \\
                \hline
                 BF    		& ${}^1\Sigma^{+}$     	& (10,8) \\
                 BH    		& ${}^1\Sigma^{+}$     	& (4,5) \\
                 C$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& (8,8) \\
                 CH$_2$ 	    & ${}^1A_{1}$         	& (6,6) \\
                 CH$_4$ 	    & ${}^1A_{1}$         	& (8,8) \\
                 CO    		& ${}^1\Sigma^{+}$     	& (10,8) \\
                 F$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& (14,8) \\
                 H$_2$O 	    & ${}^1A_{1}$         	& (8,6) \\
                 HCN    	    & ${}^1\Sigma^{+}$     	& (10,9) \\
                 HF    		& ${}^1\Sigma^{+}$     	& (8,5) \\
                 HNC        	& ${}^1\Sigma^{+}$     	& (10,9) \\
                 HNO    	    & ${}^1A^{\prime}$     	& (12,9) \\
                 HOF    	    & ${}^1A^{\prime}$     	& (14,9) \\
                 N$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& (10,8) \\
                 N$_2$H$_2$  & ${}^1A_{g}$         	& (12,10) \\
                 NH$_3$ 	    & ${}^1A_{1}$         	& (8,7) \\
                 BO    		& ${}^2\Sigma^{+}$     	& (9,8) \\
                 CH    		& ${}^2\Pi$            	& (5,5) \\
                 NH$_2$ 	    & ${}^2B_{1}$         	& (7,6) \\
                 OH    		& ${}^2\Pi$            	& (7,5) \\
                 B$_2$ 		& ${}^3\Sigma^{-}_{g}$ 	& (6,8) \\
                 CH$_2$ 	    & ${}^3B_{1}$         	& (6,6) \\
                 NF    		& ${}^3\Sigma^{-}$     	& (12,8) \\
                 NH    		& ${}^3\Sigma^{-}$     	& (6,5) \\
                 O$_2$ 		& ${}^3\Sigma^{-}_{g}$ 	& (12,8) \\
                \hline\hline
            \end{tabular}
        }
    \end{center}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bond length errors for DZ, TZ, and QZ basis.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\begin{table}

    \caption{Errors in computed equilibrium bond lengths ($\Delta \req$, pm)$^{a}$ from CI- and v2RDM-CASSCF using the cc-pVXZ (X = D, T, Q) basis sets.
    Computed bond lengths are compared to those obtained from experiment ($\req$, \AA). All values of \req were taken from Ref.~\citenum{CCCBDB} and the references  
    therein.}

    \label{tab:bond_length_errors}

    \begin{center}
        {\scriptsize
            \begin{tabular}{l c c ............. }
                \hline\hline
                & &\multicolumn{12}{c}{$\Delta \req$} \\
                \cline{5-15}
                & & & &\multicolumn{3}{c}{cc-pVDZ} &~& \multicolumn{3}{c}{cc-pVTZ} &~& \multicolumn{3}{c}{cc-pVQZ} &  \\
                \cline{5-7} \cline{9-11} \cline{13-15}
                Molecule & Term & Bond & \req & \multicolumn{1}{c}{CI} & \multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2} &~& \multicolumn{1}{c}{CI} & \multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2} &~& \multicolumn{1}{c}{CI} & \multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2}   \\
                \hline
                 BF        	& ${}^1\Sigma^{+}$ 		& B-F & 1.267 & 2.4  & 2.5 & 2.5   && 0.1  & 0.1  & 0.1  && -0.2 & -0.2 & -0.2 \\
                 BH        	& ${}^1\Sigma^{+}$ 		& H-B & 1.232 & 3.5  & 4.1 & 3.5   && 1.9  & 2.5  & 1.9  && 1.7  & 2.3  & 1.7 \\
                 C$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& C-C & 1.242 & 2.4  & 7.1 & 2.8   && 1.3  & 5.8  & 1.7  && 1.1  & 5.5  & 1.5 \\
                 CH$_2$   	& ${}^1A_{1}$ 			& H-C & 1.107 & 3.2  & 3.6 & 3.2   && 1.8  & 2.3  & 1.8  && 1.7  & 2.2  & 1.7 \\
                 CH$_4$   	& ${}^1A_{1}$ 			& H-C & 1.087 & 2.5  & 3.2 & 2.5   && 1.4  & 2.2  & 1.5  && 1.4  & 2.2  & 1.4 \\
                 CO        	& ${}^1\Sigma^{+}$ 		& C-O & 1.128 & 1.4  & 1.8 & 1.4   && 0.7  & 1.1  & 0.8  && 0.5  & 0.9  & 0.5 \\
                 F$_2$  	    & ${}^1\Sigma^{+}_{g}$ 	& F-F & 1.412 & 10.5 & 10.5 & 10.5 && 4.9  & 4.9  & 4.9  && 4.8  & 4.8  & 4.8 \\
                 H$_2$O   	& ${}^1A_{1}$ 			& H-O & 0.958 & 1.3  & 1.4 & 1.3   && 0.6  & 0.7  & 0.6  && 0.5  & 0.6  & 0.5 \\
                 HCN       	& ${}^1\Sigma^{+}$ 		& H-C & 1.064 & 2.4  & 3.0 & 2.4   && -0.7 & 1.9  & -0.7 && -0.7 & -0.6 & -0.7 \\
                           	& 						& C-N & 1.156 & 1.9  & 2.8 & 2.0   && 0.4  & 1.7  & 0.5  && 0.3  & 0.8  & 0.3 \\
                 HF        	& ${}^1\Sigma^{+}$ 		& H-F & 0.917 & 0.5  & 0.5 & 0.5   && 0.0  & 0.0  & 0.0  && -0.2 & -0.2 & -0.2 \\
                 HNC     	& ${}^1\Sigma^{+}$ 		& H-N & 0.986 & 2.5  & 3.3 & 2.5   && 1.6  & 2.4  & 1.7  && 1.6  & 2.4  & 1.6 \\
                          	& 						& C-N & 1.173 & 1.6  & 2.5 & 1.7   && 0.5  & 1.3  & 0.5  && 0.3  & 1.2  & 0.4 \\
                 HNO     	& ${}^1A^{\prime}$ 		& H-N & 1.090 & -0.2 & 0.0 & -0.2  && -1.3 & -1.1 & -1.2 && -1.4 & -1.3 & -1.3 \\
                          	& 						& N-O & 1.209 & 0.6  & 1.4 & 0.7   && 0.2  & 1.0  & 0.3  && 0.0  & 0.8  & 0.1 \\
                 HOF      	& ${}^1A^{\prime}$ 		& H-O & 0.960 & 1.9  & 2.2 & 2.0   && 1.2  & 1.4  & 1.2  && 1.0  & 1.3  & 1.1 \\
                          	& 						& O-F & 1.442 & 4.9  & 5.4 & 4.9   && 2.1  & 2.6  & 2.1  && 1.9  & 2.4  & 1.9 \\
                 N$_2$  		& ${}^1\Sigma^{+}_{g}$ 	& N-N & 1.098 & 1.9  & 2.3 & 1.9   && 0.8  & 1.3  & 0.9  && 0.6  & 1.1  & 0.7 \\
                 N$_2$H$_2$	& ${}^1A_{g}$ 			& H-N & 1.028 & 2.5  & 3.3 & 2.6   && 1.5  & 2.3  & 1.6  && 1.4  & 2.2  & 1.4 \\
                             & 						& N-N & 1.252 & 1.3  & 1.3 & 1.4   && 0.7  & 0.7  & 0.8  && 0.5  & 0.5  & 0.6 \\
                 NH$_3$    	& ${}^1A_{1}$ 			& H-N & 1.012 & 2.2  & 2.5 & 2.2   && 1.1  & 1.5  & 1.1  && 0.9  & 1.3  & 1.0 \\
                 BO          & ${}^2\Sigma^{+}$ 		& B-O & 1.204 & 1.3  & 1.9 & 1.4   && 0.9  & 1.5  & 1.0  && 0.6  & 1.2  & 0.7 \\
                 CH        	& ${}^2\Pi$ 			    & H-C & 1.120 & 2.7  & 2.5 & 2.7   && 1.3  & 1.2  & 1.3  && 1.1  & 1.0  & 1.1 \\
                 NH$_2$   	& ${}^2B_1$ 			    & H-N & 1.024 & 2.3  & 2.6 & 2.3   && 1.3  & 1.6  & 1.3  && 1.2  & 1.4  & 1.2 \\
                 OH       	& ${}^2\Pi$ 			    & H-O & 0.970 & 1.3  & 1.3 & 1.3   && 0.5  & 0.5  & 0.5  && 0.3  & 0.3  & 0.3 \\
                 B$_2$  		& ${}^3\Sigma^{-}_{g}$	& B-B & 1.590 & 3.9 & 8.2 & 4.3    && 2.7  & 7.0  & 3.1  && 2.4  & 6.7  & 2.9 \\
                 CH$_2$   	& ${}^3B_1$ 				& H-C & 1.085 & 1.7  & 1.9 & 1.7   && 0.5  & 0.7  & 0.5  && 0.4  & 0.7  & 0.4 \\
                 NF       	& ${}^3\Sigma^{-}$ 		& N-F & 1.317 & 1.7  & 1.8 & 1.7   && 0.9  & 1.0  & 0.9  && 0.8  & 0.9  & 0.8 \\
                 NH        	& ${}^3\Sigma^{-}$ 		& H-N & 1.036 & 2.3  & 2.3 & 2.3   && 1.1  & 1.1  & 1.1  && 1.0  & 1.0  & 1.0 \\
                 O$_2$  		& ${}^3\Sigma^{-}_{g}$ 	& O-O & 1.208 & 1.3  & 2.0 & 1.4   && 1.0  & 1.7  & 1.1  && 0.8  & 1.4  & 0.9 \\
                \hline                                                                                     
                            & & MSE$^b$ & - & 2.3  & 3.0  & 2.4  && 1.0 & 1.8 & 1.1 && 0.9 & 1.5 & 0.9  \\
                            & & MUE$^c$ & - & 2.3  & 3.0  & 2.4  && 1.2 & 1.8 & 1.2 && 1.0 & 1.6 & 1.1  \\
                            & & Max$^d$ & - & 10.5 & 10.5 & 10.5 && 4.9 & 7.0 & 4.9 && 4.8 & 6.7 & 4.8  \\
                \hline\hline
            \end{tabular}
        }
    \end{center}
    { \scriptsize 
        ${}^a$ $\Delta \req = \req^{\rm CASSCF} - \req$. ${}^b$ mean signed error. ${}^c$ mean unsigned error. ${}^d$ maximum unsigned error.
    }
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bond angle errors for DZ, TZ, and QZ basis.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\begin{table}

    \caption{Errors in computed equilibrium bond angles ($\Delta \aeq$, degrees)$^a$ from CI- and v2RDM-CASSCF using the cc-pVXZ (X=D,T,Q) basis sets. The cc-pVXZ-JK auxiliary basis sets were used in the v2RDM-CASSCF optimizations. Computed bond angles are compared to those obtained from experiment (\aeq, degrees). All values of \aeq were taken from Ref.~\citenum{CCCBDB} and the references therein.}

    \label{tab:angle_errors}

    \begin{center}
        {\scriptsize
            \begin{tabular}{l c c . ............ }
                \hline\hline
                & & &\multicolumn{12}{c}{$\Delta \aeq$} \\
                \cline{5-15}
                & & & &\multicolumn{3}{c}{cc-pVDZ} &~& \multicolumn{3}{c}{cc-pVTZ} &~& \multicolumn{3}{c}{cc-pVQZ} &  \\
                \cline{5-7} \cline{9-11} \cline{13-15}
                Molecule & Term & Bond & \aeq &\multicolumn{1}{c}{CI} &\multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2} & ~&\multicolumn{1}{c}{CI} &\multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2} &~&\multicolumn{1}{c}{CI}&\multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2}   \\
                \hline
                 CH$_2$  	& ${}^1A_{1}$ 		& H-C-H 	& 102.4 & -2.4 & -1.8 & -2.4 && -1.4 & -1.0 & -1.4 && -1.2 & -0.9 & -1.2 \\
                 H$_2$O   	& ${}^1A_{1}$		& H-O-H 	& 104.5 & -3.3 & -3.5 & -3.3 && -1.9 & -2.1 & -1.9 && -1.6 & -1.8 & -1.6 \\
                 HNO      	& ${}^1A^{\prime}$ 	& H-N-O 	& 108.0 &  0.5 &  1.1 &  0.5 &&  0.9 &  1.4 &  0.9 &&  1.0 &  1.5 &  1.0 \\
                 HOF      	& ${}^1A^{\prime}$ 	& H-O-F 	& 97.2  & -1.3 & -1.6 & -1.3 && -0.2 & -0.5 & -0.2 && -0.1 & -0.4 & -0.1 \\
                 N$_2$H$_2$	& ${}^1A_g$ 			& H-N-N 	& 106.3 & -1.3 & -0.1 & -1.3 && -0.6 &  0.5 & -0.7 && -0.5 &  0.7 & -0.5 \\
                 NH$_3$   	& ${}^1A_{1}$ 		& H-N-H 	& 106.7 & -3.9 & -3.6 & -3.9 && -2.1 & -2.1 & -2.1 && -1.8 & -1.7 & -1.8 \\
                 NH$_2$  	& ${}^2B_1$ 	    		& H-N-H 	& 103.4 & -3.2 & -3.1 & -3.2 && -1.9 & -2.0 & -1.9 && -1.6 & -1.7 & -1.7 \\
                 CH$_2$   	& ${}^3B_1$ 			& H-C-H 	& 135.5 & -4.5 & -4.9 & -4.5 && -4.2 & -4.5 & -4.2 && -4.2 & -4.5 & -4.2 \\
                \hline                                                                                     
                            & & MSE$^b$  & - & -2.4 & -2.2 & -2.4 && -1.4 & -1.3 & -1.5 && -1.2 & -1.1 & -1.3  \\
                            & & MUE$^c$  & - &  2.5 &  2.5 &  2.5 &&  1.7 &  1.8 &  1.7 &&  1.5 &  1.7 &  1.5  \\
                            & & Max$^d$  & - &  4.5 &  4.9 &  4.5 &&  4.2 &  4.5 &  4.2 &&  4.2 &  4.5 &  4.2  \\
                \hline\hline
            \end{tabular}
        }
    \end{center}
    { \scriptsize 
        ${}^a$ $\Delta \aeq = \aeq^{\rm CASSCF} - \aeq$. ${}^b$ mean signed error. ${}^c$ mean unsigned error. ${}^d$ maximum unsigned error.
    }
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Harmonic Frequencies
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\begin{table}

    \caption{Errors in computed harmonic vibrational frequencies ($\Delta \weq$, cm$^{-1}$)$^a$ computed using CI- and v2RDM-CASSCF for the cc-pVDZ basis set. The cc-pVDZ-JK auxiliary basis set was used for the v2RDM-CASSCF calculations. Computed frequencies are compared to those obtained from experiment (\weq, cm$^{-1}$). All values of \weq were taken from Ref.~\citenum{CCCBDB} and the references therein.}

    \label{tab:freqs}

    \begin{center}
        {\scriptsize
            \begin{tabular}{l c c c . ... }
                \hline\hline
                & & & & &\multicolumn{3}{c}{$\Delta \weq$} \\
                \cline{6-8}
                %& & & & &\multicolumn{3}{c}{cc-pVDZ}   \\
                %\cline{6-8} \\
                Molecule & Term & Mode & Sym & \weq & \multicolumn{1}{c}{CI} & \multicolumn{1}{c}{PQG} &\multicolumn{1}{c}{PQG+T2}   \\
                \hline
                 BF			& ${}^1\Sigma^{+}$ 		& 1	& $\Sigma$ 			& 1402 & -67     & -68      & -68^{b} \\
                 BH 		    & ${}^1\Sigma^{+}$ 		& 1 & $\Sigma$ 			& 2367 & -100    & -139     & -99 \\
                 C$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& 1	& $\Sigma_{\rm g}$	& 1855 & -5      & -363     & -31 \\
                 CH$_2$ 	    & ${}^1A_{1}$ 		    & 1 & A$_1$ 			    & 2806 & -14     & -45      & -16 \\
                 			&						& 2	& A$_1$				& 1353 & 64      & 9        & 64 \\
                 			&						& 3 & B$_2$				& 2865 & -11     & -19      & -12 \\
                 CH$_4$ 	    & ${}^1A_{1}$ 			& 1 & A$_1$ 			    & 2917 & 22      & -34      & 20^{b} \\
                 			&						& 2 & E 				    & 1534 & 22      & -9       & 22^{b} \\
                 			&						& 3 & T$_2$ 			    & 3019 & 49      & 66       & 48^{b} \\
                 			&						& 4 & T$_2$ 			    & 1306 & 34      & 25       & 33^{b} \\
                 CO 		    & ${}^1\Sigma^{+}$ 		& 1 & $\Sigma$ 			& 2170 & -5      & -43      & -11 \\
                 F$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& 1	& $\Sigma_{\rm g}$ 	& 917  & -304    & -305     & -304 \\
                 H$_2$O 	    & ${}^1A_{1}$ 		    & 1	& A$_1$ 			    & 3657 & 65      & 42       & 62 \\
                 			&						& 2	& A$_1$ 			    & 1595 & 121     & 114      & 121 \\
                 			&						& 3	& B$_2$ 			    & 3756 & 78      & 55       & 79 \\
                 HCN 		& ${}^1\Sigma^{+}$ 		& 1 & $\Sigma$ 			& 3312 & 59      & 7        & 55^{b} \\
                             &                  		& 2	& $\Sigma$ 			& 2089 & 6       & -65      & -4^{b} \\
                             &                  		& 3 & $\Pi$				& 712  & 10      & -107     & 7^{b} \\
                 HF 		    & ${}^1\Sigma^{+}$ 		& 1 & $\Sigma$ 			& 4138 & -83     & -83      & -83 \\
                 HNC 		& ${}^1\Sigma^{+}$ 		& 1 & $\Sigma$ 			& 3653 & 84      & -14      & 79^{b} \\
                             &                 		& 2	& $\Sigma$ 			& 2029 & 14      & -59      & 6^{b} \\
                          	&						& 3 & $\Pi$				& 477  & -1      & -245     & -5^{b} \\
                 HNO 		& ${}^1A^{\prime}$ 		& 1 & A$^{\prime}$ 		& 2684 & -48     & -26      & -54 \\
                             &                 		& 2 & A$^{\prime}$ 		& 1565 & 36      & 15       & 29 \\
                             &                 		& 3 & A$^{\prime}$ 		& 1501 & 39      & 42       & 33 \\
                 HOF 		& ${}^1A^{\prime}$ 		& 1 & A$^{\prime}$ 		& 3537 & 125     & 88       & 121^{b} \\
                             &                 		& 2 & A$^{\prime}$ 		& 1393 & -67     & -80      & -69^{b} \\
                             &                 		& 3 & A$^{\prime}$ 		& 886  & -140    & -150     & -140^{b} \\
                 N$_2$ 		& ${}^1\Sigma^{+}_{g}$ 	& 1	& $\Sigma_{\rm g}$ 	& 2359 & -4      & -54      & -15 \\
                 N$_2$H$_2$	& ${}^1A_{g}$ 			& 1 & A$_{\rm g}$ 		& 3058 & 37      & -65      & 26^{b} \\
                 			&						& 2 & A$_{\rm g}$ 		& 1583 & 37      & 30       & 35^{b} \\
                 			&						& 3 & A$_{\rm g}$ 		& 1529 & 20      & 16       & 12^{b} \\
                 			&						& 4 & A$_{\rm u}$ 		& 1289 & 27      & -10      & 25^{b} \\
                 			&						& 5 & B$_{\rm u}$ 		& 3120 & 3       & -73      & -5^{b} \\
                 			&						& 6 & B$_{\rm u}$ 		& 1316 & 37      & 28       & 35^{b} \\
                 NH$_3$ 	    & ${}^1A_{1}$ 		    & 1 & A$_1$ 			    & 3337 & -9      & -72      & -36 \\
                 			&						& 2 & A$_1$ 			    & 950  & 279     & 129      & 149 \\
                 			&						& 3 & E 				    & 3444 & 8       & 3        & 12 \\
                 			&						& 4 & E 				    & 1627 & 81      & 54       & 71 \\
                 BO 		    & ${}^2\Sigma^{+}$ 		& 1	& $\Sigma$ 			& 1886 & -14     & -61      & -19^{b} \\
                 CH 		    & ${}^2\Pi$ 			    & 1	& $\Sigma$ 			& 2859 & -114    & -83      & -114^{b} \\
                 NH$_2$ 	    & ${}^2B_1$ 			    & 1	& A$_1$ 			    & 3219 & -5      & -30      & -7^{b} \\
                 			&						& 2	& A$_1$ 			    & 1497 & 76      & 68       & 76^{b} \\
                 			&						& 3	& B$_2$ 			    & 3301 & 6       & -19      & 5^{b} \\
                 OH 		    & ${}^2\Pi$ 			    & 1	& $\Sigma$ 			& 3738 & -130    & -130     & -130 \\
                 B$_2$ 		& ${}^3\Sigma^{-}_{g}$	& 1	& $\Sigma_{\rm g}$ 	& 1051 & -32     & -173     & -51 \\
                 CH$_2$ 	    & ${}^3B_1$			    & 1 & A$_1$				& 2806 & 245     & 218      & 245^{b} \\
                 			&						& 2 & A$_1$				& 963  & 160     & 193      & 160^{b} \\
                 			&						& 3 & B$_2$				& 3190 & 71      & 42       & 70^{b} \\
                 NF 		    & ${}^3\Sigma^{-}$ 		& 1 & $\Sigma$ 			& 1141 & -65     & -67      & -66^{b} \\
                 NH 		    & ${}^3\Sigma^{-}$ 		& 1	& $\Sigma$ 			& 3282 & -171    & -171     & -171 \\
                 O$_2$ 		& ${}^3\Sigma^{-}_{g}$ 	& 1	& $\Sigma_{\rm g}$	& 1580 & -51     & -108     & -62^{b} \\
                \hline                                                                                     
                            & & & MSE$^c$ & - & 9   & -33  & 2  \\
                            & & & MUE$^d$ & - & 64  &  81  & 63  \\
                            & & & Max$^e$ & - & 304 & 363  & 304  \\
                \hline\hline
            \end{tabular}
        }
    \end{center}
    { \scriptsize 
        ${}^a$ $\Delta \weq = \weq^{\rm CASSCF} - \weq$. ${}^b$ ``loose'' convergence criteria used (Sec.~\ref{SEC:DETAILS}). ${}^c$ mean signed error. ${}^d$ mean unsigned error. ${}^e$ maximum unsigned error.
    }
\end{table}








